Butterfly-Core Community Search over Labeled Graphs

Community search aims at finding densely connected subgraphs for query vertices in a graph. While this task has been studied widely in the literature, most of the existing works only focus on finding homogeneous communities rather than heterogeneous communities with different labels. In this paper, we motivate a new problem of cross-group community search, namely Butterfly-Core Community (BCC), over a labeled graph, where each vertex has a label indicating its properties and an edge between two vertices indicates their cross relationship. Specifically, for two query vertices with different labels, we aim to find a densely connected cross community that contains two query vertices and consists of butterfly networks, where each wing of the butterflies is induced by a k-core search based on one query vertex and two wings are connected by these butterflies. Indeed, the BCC structure admits the structure cohesiveness and minimum diameter, and thus can effectively capture the heterogeneous and concise collaborative team. Moreover, we theoretically prove this problem is NP-hard and analyze its non-approximability. To efficiently tackle the problem, we develop a heuristic algorithm, which first finds a BCC containing the query vertices, then iteratively removes the farthest vertices to the query vertices from the graph. The algorithm can achieve a 2-approximation to the optimal solution. To further improve the efficiency, we design a butterfly-core index and develop a suite of efficient algorithms for butterfly-core identification and maintenance as vertices are eliminated. Extensive experiments on eight real-world networks and four novel case studies validate the effectiveness and efficiency of our algorithms.

==> content/sec-exp-old.tex <==
In this section, we introduce the experiments based on $7$ real-world networks where all networks are treated as undirected, including $2$ enterprise communication network from one Internet technology company in China namely Company-Quarter and Company-Year, $5$ synthetic network constructed from public SNAP dataset~\footnote{http://snap.stanford.edu/data/}, namely Amazon, DBLP, Youtube, LiveJournal and Orkut. The network statistics are shown in Table~\ref{snap}. Due to the same trend of results and the space limitation, in some experiments we only show the results of some representative datasets.

%Particularly, to facilitate the readability and reproducibility, the details of our experimental setup, including dataset preprocessing, evaluation metrics, and parameter settings, are introduced in appendix as supplementary information.

%%
%% If your work has an appendix, this is the place to put it.
% \appendix
% cat /proc/cpuinfo
% lscpu
In our experiments, all the algorithms were implemented with C++ and conducted on a Linux Server with Intel Xeon CPU $E5-2620$ ($2.20$ GHz) and $125$ GB main memory.

\begin{table}[th]
\centering
\small
\vspace{-0.2cm}
\caption{Network statistics $(K = 10^3$ and $M = 10^6)$.}
\label{snap}
%\vspace{-0.2cm}
\begin{tabular}{ l|rrrrr }
\hline
{\bf Network} & $|V_G|$ & $|E_G|$ & $Labels$ & $k_{max}$ & $d_{max}$  \\
 \hline
%Facebook  & 4\bf{K} & 88\bf{K} \\
Company-Quarter & 30\bf{K} & 508\bf{K} & 200  & 43 & 11\\
Company-Year & 41\bf{K} & 2\bf{M} & 200  & 189 & 11\\
Amazon  & 335\bf{K} & 926\bf{K} & 2  & 6 & 549\\
DBLP  & 317\bf{K} & 1\bf{M} & 2  & 113 & 342\\
Youtube & 1.1\bf{M} & 3\bf{M} & 2  & 51 & 28,754\\
LiveJournal & 4\bf{M} & 35\bf{M} & 2  & 360 &14,815\\
Orkut & 3.1\bf{M} & 117\bf{M} & 2  & 253 & 33,313\\ \hline
\end{tabular}
\vspace{-0.2cm}
\end{table}

\subsection{Experimental Setup}

In the two company network dataset, each node represents an employee, label represents the department of the employee and an edge exists between two employees if they have communicated through the company inner instant messaging software. The ground truth communities are the joint projects among two teams from different departments of companies. Company-Quarter dataset is a collection for three consecutive months and Company-Year consists of data in one whole year. Considering the temporary chat, we set a threshold as $20$ and $5$ respectively for Company-Year and Company-Quarter, then filter the edges if the weight less than the threshold. For the other $5$ snap networks we need add some synthetic information to fit our studied problem settings. 

\vspace{-0mm}
\spara{SNAP Network Construction.} Indeed, the nodes on the SNAP original network do not have labels and there may not be edges across two communities. Therefore, we added new information for the network to fit our problem in the following steps:
\squishlisttight
\vspace{-1mm}
\item \spara{Add node labels}. We split the \textbf{w}hole \textbf{g}round \textbf{t}ruth \textbf{c}ommunities (wgtc) by communities into $t$ parts, assigning all the nodes in each part with one label. Here we set $t = 2$ which is the most challenging case when the size of the subgraph of one label is maximized. Since one node may have more than one community, if these communities appear in different parts, the nodes label will be randomly assigned. There are also very less nodes on the graph (less than $5\%$) having no communities whose labels are also randomly assigned. The community label is dominated by the majority label of its nodes.

\vspace{-1mm}
\item \spara{Generate qualified query pairs for test}. Considering the quality of communities, we selected the evaluated query pairs from the nodes shown in the \textbf{t}op \textbf{5}k \textbf{c}ommunities (t5c). We iterated the nodes in t5c and then picked out the nodes that have and only have one community in wgtc, generating the nodes set $S$. We then generate the query node pairs from $S$ by picking any two nodes with different labels.

\vspace{-1mm}
\item \spara{Add cross edges between test communities}. The generation way of query node pairs guarantees there is only one community including each query node and it is a top 5k community. For two communities of the test query node pair, we first randomly picked two nodes and add cross edges to make them contain $5$ butterflies and then randomly added 10\% cross edges between the two communities to simulate the collaboration across teams. Globally we also randomly added 10\% cross edges in the bipartite graph between two labeled subgraph.
\end{list}

\begin{figure}[t!]
%\small
\vspace{-5mm}
\centering
%\includegraphics[width=0.7\linewidth,natwidth=400,natheight=310]{./exp/f1.pdf}
\includegraphics[width=0.7\linewidth]{./exp/aggreg.eps}
\vspace{-5mm}
\caption{Quality evaluation (F1 score) on networks with ground-truth communities}
\vspace{-6mm}
\label{fig.f1}
\end{figure}


 %In addition, to evaluate the quality of the detected butterfly-core community, we implemented two classical community search methods: 1) $k$-core, which finds the dense subgraph where the degree of each node is no less than $k$; and 2) $k$-truss, where each edge has a support no less than $k - 2$, for both methods we add the same minimize diameter constraint.

\spara{Metric.}
For evaluating efficiency, we report the running time in seconds. We treat the running time of a query as infinite if it exceeds $30$ minutes. We test the datasets with ground-truth, and show the F1-score to measure the alignment between a discovered community $C$ and a ground-truth community $\hat{C}$. Here, F1 is defined as $F1(C, \hat{C}) = \frac{2·prec(C, \hat{C})·recall(C, \hat{C})}{prec(C, \hat{C}) + recall(C, \hat{C})}$ where $prec(C, \hat{C}) = \frac{|C \cap \hat{C}|}{|C|}$ is precision and $recall(C, \hat{C}) = \frac{|C \cap \hat{C}|}{|\hat{C}|}$ is recall.

\spara{Query pairs parameters.}
Two parameters, degree rank $Q_d$ and inter-distance $l$ are varied for selecting different sets of query nodes. Here, $Q_d$ is the degree rank of query nodes. We sorted all vertices in ascending order of their degrees in a network. A node is regarded to be with degree rank of $X\%$, if it has top highest $X\%$ degree in the network. The default value of $Q_d$ is $80\%$, which means that a query node has degree higher than the degree of $80\%$ nodes in the whole network. The inter-distance $l$ is the inter-distance between two query nodes. The default $l = 1$ indicates that the two query nodes are directly connected in the network. 
%In summary, the default value of $Q_d$ is $80\%$ and the default distance $l$ is $l = 1$.


%test 202007
%\begin{figure*}
%  \includegraphics[width=\textwidth,natwidth=1800,natheight=310]{./figures_exp/6.pdf}
%  \caption{The framework overview of our MANE approach.}
%  \label{framework}
%\end{figure*}


%\begin{figure*}[t]
%\small
%%\vspace{-7mm}
%\centering
%%\includegraphics[width=\linewidth,natwidth=1500,natheight=600]{./fig_exp/24_2.pdf}
%\includegraphics[width=\linewidth]{./fig_exp/tmp.pdf}
%%\vspace{-7mm}
%\caption{Varying node degree rank: Query Time}
%\vspace{-3mm}
%\label{fig.d}
%\end{figure*}


%htp
\begin{figure*}[t]
%\vspace*{-0.5cm}
\centering \mbox{
\subfigure[Company-Quarter]{\includegraphics[width=0.2\linewidth]{./vary/degree1.eps}}%\hskip 0.2in
\subfigure[Company-Year]{\includegraphics[width=0.2\linewidth]{./vary/degree2.eps}} %\hskip 0.2in
\subfigure[DBLP]{\includegraphics[width=0.2\linewidth]{./vary/degree3.eps}}%\hskip 0.2in
\subfigure[LiveJournal]{\includegraphics[width=0.2\linewidth]{./vary/degree4.eps}} %\hskip 0.2in
\subfigure[Orkut]{\includegraphics[width=0.2\linewidth]{./vary/degree5.eps}} %\hskip 0.2in
\vspace*{-0.5cm}
}
\vspace*{-0.5cm}
\caption{Varying node degree rank: Query Time}
\vspace*{-0.4cm}
\label{fig.d}
\end{figure*}
%test 202007


%htp
\begin{figure*}[t]
%\vspace*{-0.5cm}
\centering \mbox{
\subfigure[Company-Quarter]{\includegraphics[width=0.2\linewidth]{./fig_exp/test27-2.eps}}%\hskip 0.2in
\subfigure[Company-Year]{\includegraphics[width=0.2\linewidth]{./fig_exp/test27-2.eps}} %\hskip 0.2in
\subfigure[DBLP]{\includegraphics[width=0.2\linewidth]{./fig_exp/test27-2.eps}}%\hskip 0.2in
\subfigure[LiveJournal]{\includegraphics[width=0.2\linewidth]{./fig_exp/test27-2.eps}} %\hskip 0.2in
\subfigure[Orkut]{\includegraphics[width=0.2\linewidth]{./fig_exp/test27-2.eps}} %\hskip 0.2in
\vspace*{-0.5cm}
}
\vspace*{-0.5cm}
\caption{Varying inner distance l: Query Time}
\vspace*{-0.4cm}
\label{fig.l}
\end{figure*}
%test 202007


%htp
\begin{figure*}[t]
%\vspace*{-0.5cm}
\centering \mbox{
\subfigure[Company-Quarter]{\includegraphics[width=0.2\linewidth]{./vary/k1.eps}}%\hskip 0.2in
\subfigure[Company-Year]{\includegraphics[width=0.2\linewidth]{./vary/k2.eps}} %\hskip 0.2in
\subfigure[DBLP]{\includegraphics[width=0.2\linewidth]{./vary/k3.eps}}%\hskip 0.2in
\subfigure[LiveJournal]{\includegraphics[width=0.2\linewidth]{./vary/k4.eps}} %\hskip 0.2in
\subfigure[Orkut]{\includegraphics[width=0.2\linewidth]{./vary/k5.eps}} %\hskip 0.2in
\vspace*{-0.5cm}
}
\vspace*{-0.5cm}
\caption{Varying core value k: Query Time}
\vspace*{-0.4cm}
\label{fig.k}
\end{figure*}
%test 202007


%htp
\begin{figure*}[t]
%\vspace*{-0.5cm}
\centering \mbox{
\subfigure[Company-Quarter]{\includegraphics[width=0.2\linewidth]{./vary/b1.eps}}%\hskip 0.2in
\subfigure[Company-Year]{\includegraphics[width=0.2\linewidth]{./vary/b2.eps}} %\hskip 0.2in
\subfigure[DBLP]{\includegraphics[width=0.2\linewidth]{./vary/b3.eps}}%\hskip 0.2in
\subfigure[LiveJournal]{\includegraphics[width=0.2\linewidth]{./vary/b4.eps}} %\hskip 0.2in
\subfigure[Orkut]{\includegraphics[width=0.2\linewidth]{./vary/b5.eps}} %\hskip 0.2in
\vspace*{-0.5cm}
}
\vspace*{-0.5cm}
\caption{Varying butterfly value b: Query Time}
\vspace*{-0.4cm}
\label{fig.b}
\end{figure*}
%test 202007


\subsection{Quality and Efficiency Evaluation}
To the best of our knowledge, there is no related work to handle our studied community. To evaluate the quality found by the Butterfly-Core Community model, we select two state-of-the-art community search methods as benchmarks.

\squishlisttight
\item CTC: \textbf{C}losest \textbf{C}ommunity \textbf{S}earch which finds a closest truss community containing query set \citep{huang2015approximate}.

\item PSA: \textbf{P}rogressive \textbf{S}earch \textbf{A}lgorithm which finds a minimum $k$-core containing query set \citep{li2019efficient}.

\end{list}

We compared the baselines with three of our approaches as following: %Algorithm~\ref{algo:sssp} and Algorithm~\ref{algo:LeaderPair}:
\squishlisttight

\item BD: the method of Butterfly-Core Community online search in Algorithm \ref{algo:Basic} using \textbf{B}ulk \textbf{D}eletion that removes a batch of vertices with the furthest distances from graph.

\item BDQL: the \textbf{B}ulk \textbf{D}eletion method with two accelerate strategies, i.e. Fast \textbf{Q}uery Distance Computation in Algorithm~\ref{algo:sssp} and \textbf{L}eader Pair in Algorithm~\ref{algo:LeaderPair}.  


\item LBCC: the \textbf{L}ocal search based \textbf{B}utterfly-\textbf{C}ore \textbf{C}ommunity method with Bulk Deletion, Algorithm~\ref{algo:sssp} and \ref{algo:LeaderPair}.
\end{list}

%For effectiveness and efficiencies we select different baselines to test, i.e. effectiveness with $k$-truss and $k-$core; efficiencies with BD.

\spara{Model Parameters setting.}
For all the butterfly-core based models, i.e., BD, BDQL and LBCC, we set $k_1$ and $k_2$ as the maximum core value of query nodes $q_l$ and $q_r$ could reach respectively. Note that this setting may not reach the best F1-score but it is reasonable for the users convenience especially when the users have no sense about the graph or query nodes. For $b$, we set $b = 1$. For LBCC, we select $\gamma_1 = 0.5$ and $\gamma_2 = 0.5$. For the baselines, in the original CTC model \citep{huang2015approximate} it also picked the largest truss value $k$ the query set exist in, for the PSA model \citep{li2019efficient} we follow the same setting to set $k$ as the maximum core value.
%  query set exist in


\spara{Ground-truth Evaluation.}
To evaluate the effectiveness of different models, we compare BDQL, LBCC with baselines CTC \citep{huang2015approximate} and PSA \citep{li2019efficient} based on ground-truth communities~\citep{yang2015defining}. We randomly selected query nodes that appear in a unique ground-truth community, and selected $1,000$ sets of such query node pairs. We evaluate the accuracy of the detected communities with F1-score. Figure~\ref{fig.f1} shows the averaged F1-score on $7$ networks. We observe that our approaches can achieve the highest F1-score on most networks. Moreover, due to the large overlap of ground-truth communities~\citep{yang2015defining} in Orkut, all the approaches cannot have good detection results compared with other datasets.
%while $k$-truss outperforms $k-$core slightly since it may find a denser graph


%Due to the space limitation we use these 3 to show and included the largest netwrok Orkut we have.
\spara{Efficiency Evaluation.}
To evaluate the efficiency of improved strategies, we test BD, BDQL, and LBCC algorithms proposed in this paper. Here, we use BD as the baseline but not Basic since the Basic approach in Algorithm~\ref{algo:Basic} is too time-consuming and mostly cannot finish in $30$ minutes. Figure~\ref{fig.d} and Figure~\ref{fig.l} show the running time on different networks, varying the node degree rank and inner distance respectively. We could find the most efficiency method is LBCC since its initiated graph $G_0$ is the smallest compared with BDQL, and it is the only method which could find the answer on Orkut in $30$ minutes (around $1$ second). Increasing the node degree, we could find BD and BDQL in DBLP and LiveJournal become faster since the nodes with higher degree have denser and smaller induced graphs; it is different in the Company-Quarter and Company-Year dataset because the largest denseness of the graph e.g. largest $k$ value among these datasets. Increasing the query nodes distance $l$, the running time also slows down which may cause by the fact that two query nodes do not have direct connections, i.e. they do not play as the leaders then the leader strategy may become slower to find the true leaders.

% Index is the butterfly core index maintenance method. Mix is Basic with all the above strategies, i.e. BD, SSSP, Pair, Index and Mix.

\subsection{Parameter Sensitivity Evaluation}
%\spara{Exp-3 Parameters Sensitivity}
In the Butterfly-Core Community model, there are three parameters $\{k_1, k_2, b\}$. Here we test the influence of parameters on the algorithm running time. When analysing one parameter we will fix the other two, and we only analyse one of $\{k_1, k_2\}$ due to the symmetry property. Figure~\ref{fig.k} shows the running time on different networks, by varying the core value $k$. We observe that the larger $k$ results in the less running time, since larger $k$ could generate a smaller initial graph $G_0$. Figure~\ref{fig.b} shows the running time on different networks, by varying the butterfly value $b$. We observe that the larger $b$ results in slight less running time, due to its early stop criteria caused by the high butterfly requirement.

\subsection{Case Study}
%\subsection{Case Study on Harry Potter Network}
%\spara{Exp-4 A Case Study on Harry Potter}
Besides the evaluation on effectiveness and efficiencies, we applied our BDQL algorithm on $3$ real public networks, i.e. a global flight network~\footnote{https://openflights.org/}, an international trade network~\footnote{https://wits.worldbank.org/} and the J. K. Rowling's Harry Potter series fiction network~\footnote{https://github.com/efekarakus/potter-network}. These further evaluate the difference of our model with previous studies, w.l.o.g. we pick CTC algorithm \citep{huang2015approximate} as the baseline. We pick $k_1, k_2$ values as the maximum core value of each query node and set $b = 1$. 

The flight network is a $256$-labeled graph, each node represents a city, label represents the home country of the city and an edge is drawn between two cities if there's at least one airline between them. We want to find the dense flight transportation network of two counties Canada and Germany, then input queries with $\{Toronto, Frankfut\}$, Figure~\ref{fig.case}(a) is our community result which consists of air transport hubs, domestic and transnational airlines. Most cities our model retrived are developed cities since the large population, economic and cultural exchange have promoted cities to open airlines. Figure~\ref{fig.case}(b) is the community returned by CTC \citep{huang2015approximate}. By comparison we could find the advantages of our proposed models, we aim to mine out the whole dense teams but not only the leaders with cross edges, since some team members even without cross communications also play an important role with strong support or skeleton of the team considering it forms the dense inner team. Simply ignoring the labels and running some community search methods \citep{huang2015approximate} \citep{li2019efficient} as a whole compared with running them separately on each label graph makes a huge difference: (1) it ignores the different dense level of two teams; (2) it confuses the semantics of edge types between same labels and across labels; (3)it adds the neighbors from different labels into the node degree then the graph size constraint may result in the community to shrink then only keep some cross nodes but miss some innner members.
 
The trade network is a $7$-labeled graph, each node represents a country, the country's label is its located continent, one edge $(i, j)$ exists means country $i$ is either a top $5$ export trade partner or a top $5$ import trade partner in the year 2019. Consider the background of trade war, we input queries $\{China, US\}$, from Figure \ref{fig.case}(c) we find the dense trade network of each continent, China and US are the trade leaders in each continent, who have the most transcontinental trades. Figure \ref{fig.case}(d) is the community got from CTC \citep{huang2015approximate} which suffers the same problem, it fails to find the other main trade partners in Asia. 

The Harry Potter network is a $2$-labeled graph, where each vertex represents a character, the character's label represents his camp justice or evil, edges between two characters means they have intersections in the fiction, edges in the same camp denote the family and ally, while edges in different camp denote hostility enemies. The sample query is \{``Ron Weasley'', ``Draco Malfoy''\}. In Figure \ref{fig.case}(f) CTC \citep{huang2015approximate} only finds out Ron with his best friend of Harry and Hermione in the Gryffindor house, Malfoy and his two cronies belonging in the Slytherin house. However it misses the main leader in the evil camp, i.e. ``Lord Voldemort''. What's more, it also fails to find Ron's huge family, include his parents, brothers .etc. The result of our model is shown in Figure~\ref{fig.case}.

%Though Snape killed Dumbledore, they have positive relationship in the dataset.
%The two queries are related to the story in ``Harry Potter and the Prisoner of Azkaban'' when Harry found the truth is Peter betrays James and Lily Potter but not his godfather Sirius.
%where blue left part is dense but red right part is sparse that is a $2$-core. Indeed, it validates the ability of our model, since in the dataset Peter has many enemies but less friends.


%group 1
%\begin{figure*}[htp]
%\vspace*{-0.5cm}
%\centering \mbox{
%\subfigure[Flight]{\includegraphics[width=0.5\linewidth, height=2.5cm]{./fig_case_study/airport2.pdf}}%\hskip 0.2in
%\subfigure[Flight CTC]{\includegraphics[width=0.5\linewidth, height=2.5cm]{./fig_case_study/airport1.pdf}} %\hskip 0.2in
%\vspace*{-0.5cm}
%}
%%\vspace*{-0.5cm}
%\centering \mbox{
%%\vspace*{-8mm}
%\subfigure[Trade]{\includegraphics[width=0.5\linewidth, height=2.5cm]{./fig_case_study/trade2.pdf}}
%\subfigure[Trade CTC]{\includegraphics[width=0.5\linewidth, height=2.5cm]{./fig_case_study/trade1.pdf}}
%}
%\centering \mbox{
%\subfigure[Harry Potter]{\includegraphics[width=0.5\linewidth, height=2.5cm]{./fig_case_study/harry2.pdf}}%\hskip 0.2in
%\subfigure[Harry Potter CTC]{\includegraphics[width=0.5\linewidth, height=2.5cm]{./fig_case_study/harry1.pdf}} %\hskip 0.2in
%}
%\vspace*{-0.5cm}
%\caption{Case study on $3$ real networks: BDQL vs. CTC} \label{fig.case}
%\vspace*{-0.4cm}
%\end{figure*}


%group 2
%\begin{figure}[t]
%%\small
%%\vspace{-7mm}
%\centering
%%\includegraphics[width=0.8\linewidth,natwidth=400,natheight=270]{./exp/case.pdf}
%\includegraphics[width=0.8\linewidth]{./fig_case_study/case.pdf}
%\vspace{-4mm}
%\caption{Harry Potter case study.}
%\vspace{-6mm}
%\label{fig.case}
%\end{figure}


%\begin{figure*}[htp]
%\vspace*{-0.5cm}
%\centering \mbox{
%\subfigure[Flight]{\includegraphics[width=0.33\linewidth]{./fig_case_study/airport2.pdf}}%\hskip 0.2in
%\subfigure[Trade]{\includegraphics[width=0.33\linewidth]{./fig_case_study/trade2.pdf}} %\hskip 0.2in
%\subfigure[Harry Potter]{\includegraphics[width=0.33\linewidth]{./fig_case_study/harry2.pdf}}%\hskip 0.2in
%\vspace*{-0.5cm}
%}
%%\vspace*{-0.5cm}
%\centering
%\mbox{
%%\vspace*{-8mm}
%\subfigure[Flight CTC]{\includegraphics[width=0.33\linewidth]{./fig_case_study/airport1.pdf}}
%\subfigure[Trade CTC]{\includegraphics[width=0.33\linewidth]{./fig_case_study/trade1.pdf}}
%\subfigure[Harry Potter CTC]{\includegraphics[width=0.33\linewidth]{./fig_case_study/harry1.pdf}}
%}
%\vspace*{-0.5cm}
%\caption{Case study on $3$ real networks: BDQL vs. CTC} \label{fig.case}
%\vspace*{-0.4cm}
%\end{figure*}




%\begin{figure*}[htp]
%\vspace*{-0.5cm}
%\centering \mbox{
%\subfigure[Flight]{\includegraphics[width=0.7\linewidth, height=3.8cm]{./fig_case_study/trade2.pdf}}%\hskip 0.2in
%\subfigure[Trade]{\includegraphics[width=0.3\linewidth, height=3.8cm]{./fig_case_study/trade1.pdf}} %\hskip 0.2in
%\vspace*{-0.5cm}
%}
%\caption{test}
%\vspace*{-0.4cm}
%\end{figure*}


%group 3
%\begin{figure*}[htp]
%%\vspace*{-0.5cm}
%\centering \mbox{
%\subfigure[Flight]{\includegraphics[width=0.30\linewidth, height=3.5cm]{./fig_case_study/airport2.pdf}}%\hskip 0.2in
%\subfigure[Trade]{\includegraphics[width=0.24\linewidth, height=3.5cm]{./fig_case_study/airport1.pdf}} %\hskip 0.2in
%\subfigure[Harry Potter]{\includegraphics[width=0.46\linewidth, height=3.5cm]{./fig_case_study/trade2.pdf}}%\hskip 0.2in
%\vspace*{-0.5cm}
%}
%%\vspace*{-0.5cm}
%\centering
%\mbox{
%%\vspace*{-8mm}
%\subfigure[Flight CTC]{\includegraphics[width=0.28\linewidth, height=3.5cm]{./fig_case_study/d_trade_2.pdf}}
%\subfigure[Trade CTC]{\includegraphics[width=0.44\linewidth, height=3.5cm]{./fig_case_study/harry2.pdf}}
%\subfigure[Harry Potter CTC]{\includegraphics[width=0.28\linewidth, height=3.5cm]{./fig_case_study/harry1.pdf}}
%}
%\vspace*{-0.5cm}
%\caption{Case study on $3$ real networks: BDQL vs. CTC} \label{fig.case}
%\vspace*{-0.4cm}
%\end{figure*}


%group 4
\begin{figure}[htp]
\vspace*{-0.5cm}
\centering \mbox{
\subfigure[Flight BDQL]{\includegraphics[width=0.65\linewidth, height=2.5cm]{./fig_case_study/air2.pdf}}%\hskip 0.2in
\subfigure[Flight CTC]{\includegraphics[width=0.35\linewidth, height=2.5cm]{./fig_case_study/air1.pdf}} %\hskip 0.2in
\vspace*{-0.5cm}
}
%\vspace*{-0.5cm}
\centering \mbox{
%\vspace*{-8mm}
\subfigure[Trade BDQL]{\includegraphics[width=0.65\linewidth, height=2.5cm]{./fig_case_study/trade2.pdf}}
\subfigure[Trade CTC]{\includegraphics[width=0.35\linewidth, height=2.5cm]{./fig_case_study/trade1.pdf}}
}
\centering \mbox{
\subfigure[Harry Potter BDQL]{\includegraphics[width=0.65\linewidth, height=2.5cm]{./fig_case_study/harry2.pdf}}%\hskip 0.2in
\subfigure[Harry Potter CTC]{\includegraphics[width=0.35\linewidth, height=2.5cm]{./fig_case_study/harry1.pdf}} %\hskip 0.2in
}
\vspace*{-0.5cm}
\caption{Case study on $3$ real networks: BDQL vs. CTC} \label{fig.case}
\vspace*{-0.4cm}
\end{figure}



==> content/sec-fast_old.tex <==
%%%%%%%%%%%%%%DSSSP%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\small
\caption{Fast Query Distance Computation$(G_i, q, D_i)$} \label{algo:sssp}
\begin{algorithmic}[1]
\REQUIRE A graph  $G_i$, query node $q$, a set of removal vertices $D_i$
\ENSURE the updated distance $dist(v, Q)$ for all vertices $v$
\STATE remove all vertices $D_i$ and their incident edges from $G_i$;
%\STATE $d = dist(S.iterator.next())$;
\STATE $d_{min} \gets min_{u \in D_i} dist(u, q)$;
% \FORALL{$v \in S$}
%     \STATE $dist.remove(v)$; $hm[dist[v]].remove(v)$;
% \ENDFOR
% \STATE $S_u \gets \emptyset$;
% \FORALL{$i \in hm.keys()$ and $i > d$}
%     \STATE $S_u \gets S_u \cup \{hm[i]\}$;% mark S_u as unvisited
% \ENDFOR
\STATE $S_s = \{v\in V(G_i)\setminus D_i | dist_{G_i}(v, Q) = d_{min} \}$;
\STATE $S_u = \{v\in V(G_i)\setminus D_i | dist_{G_i}(v, Q) > d_{min} \}$;
% \STATE $Q \gets queue$;
% \STATE $S_s \gets hm[d]$;
% \FORALL{$s \in S_s$}
%     \STATE $Q.enqueue(s)$; \label{line:a11}
% \ENDFOR
\STATE apply the BFS traverse on $G_i$ starting from $S_s$ to update the query distance of nodes in $S_u$;
\STATE return all updated distance $dist(u, q)$ for $u \in S_u$; \label{line:a22}
\end{algorithmic}
\end{algorithm}


%From the complexity analysis of Algorithm~\ref{algo:Basic}, we could find the bottlenecks are the shortest path and butterfly counting. In section \ref{sub-sec:sp} we propose a new shortest path algorithm that only update the nodes whose shortest path changed to shrink the search space. In section \ref{sub-sec:lp} we spotlight a leader pair instead of the butterfly counting on all nodes. In section \ref{sub-sec:lc} we create a local search method based on Steiner tree to find BCC.

In this section, on top of our greedy algorithmic framework in Algorithm~\ref{algo:Basic}, we propose three methods for fast BCC search. The first method is the fast computation of query distance, which only updates a partial of vertices with new query distances in Section \ref{sub-sec:sp}. The second method identifies a pair of leader vertices, which both have the butterfly degrees no less than $b$ in BCC as shown in Section \ref{sub-sec:lp}. This leader pair trends to have large butterfly degrees even after the phase of graph removal, which can 
%reduce unnecessary butterfly counting.
save lots of computations in butterfly counting.
% for nodes over an entire graph. 
The third method of local BCC search is presented in Section \ref{sub-sec:lc}, which finds a small candidate graph for bulk removal refinement, instead of starting from whole graph $G$. 

%Besides, we create offline $k$-core index for nodes, then improve the efficiency to find the $k$-core subgraph from $G$. What's more, when constructing $B$ it also filter out the edges, $(v_i, v_j),  (k_i, k_j)$. The edge set whose index holds either $k_i < k_1$ or $k_j < k_2$ initially will be excluded from the bipartite graph.

%Besides, we create offline $k$-core index for nodes which benefit for the construction of $k$-core. The retrieve of cross-group edges based on the maximum core value of two endpoints i.e. $(k_i, k_j)$. The edge set whose index holds either $k_i < k_1$ or $k_j < k_2$ initially will be excluded from the bipartite graph.

% \subsection{Bulk Deletion}
% In this subsection, we propose a similar algorithm called BulkDelete in \citep{huang2015approximate} following the framework of Algorithm~\ref{algo:Basic}, which is based on deletion of a set of nodes in batch when maintaining a butterfly-core. Since $dist_{G_i}(u, Q)$ is monotone non-decreasing with decreasing graphs, i.e., $dist_{G_j}(u, Q) \geq dist_{G_i}(u, Q) = d$, for $j > i$. Thus remove $S = \{u^\ast|dist_{G_i} (u^\ast, Q) \geq d, u^\ast \in G_i\}$ instead of single node $u^\ast$ in line \ref{line:a7} of Algorithm~\ref{algo:Basic}. However, in theory, it is possible that $|S| = 1$ in every iteration.

% Based on $dist_{G_i} (u^\ast , Q) = d$ has at least $k - 1$ neighbors $v$ with $dist_{G_i}(v, Q) \geq d - 1$ (need to check). If we remove $S = \{u^\ast|dist_{G_i} (u^\ast, Q) \geq d - 1, u^\ast \in G_i\}$ at each iteration, then at least $k$ nodes are removed each time. It can terminate quicker than Algorithm~\ref{algo:Basic}, i.e. the number of iterations is improved from $O(min\{n, m/min\{k_1, k_2\}\})$ to $O(min\{n/min\{k_1, k_2\}\})$.

% \begin{theorem}
% Algorithm BulkDelete takes $O(t ( \sum\nolimits_{u \in V} {d_u^2} + m))$ time, where $t \in O(min\{n/min\{k_1, k_2\}\})$.
% \end{theorem}

% \begin{theorem}
% Algorithm BulkDelete is a $(2 + \epsilon)$-approximation solution of BCC-Problem, where $\epsilon = 2/diam(H^\ast$).
% \end{theorem}

%In the following all of our proposed strategies
\vspace{-1mm}
\subsection{Fast Query Distance Computation}\label{sub-sec:sp}
%\subsection{Query Distance Shortest Path}\label{sub-sec:sp}
%In Algorithm~\ref{algo:Basic}, after nodes deletion we run shortest path algorithm again which is costly since all nodes are calculated. However, only a small part of nodes have been removed and the distance of most nodes on the graph to the queries don't change. Next we'll propose a method that only performs BFS on the entire graph once then updates partially. We use $q$ and $S$ to represent the query node and removing nodes set respectively. First we run the naive single source shortest path algorithm starting from $q$ in a BFS manner until visiting all the nodes and maintain two hashtables $dist$ and $hm$, $dist$ is to keep all the nodes and their shortest path value to $q$, $hm$ is to keep the shortest path value to $q$ and a nodes set with the corresponding value. To use $hm[d]$ we could get all the nodes whose shortest path to $q$ is $d$. 
%Meanwhile we maintain a integer max to keep the maximum distance storing in the current hashmap $dist$.

Here, we present a fast algorithm to compute the query distance for vertices in $G$. In the line $4$ of Algorithm~\ref{algo:Basic}, it needs to compute the query distance for all vertices, which invokes expensive computation costs. However, we observe that a majority of vertices keeps the query distance unchanged after each graph removal. This suggests that a partial update of query distances may ensure the updating exactness and speedup the efficiency. 

The key idea is to identify the vertices whose query distances need to update. Given a set of vertices $D_i$ deleted in graph $G_i$, let be the distance $d_{min}= \min_{v\in D_i} dist_{G_i}(v, Q)$. Let $S_u = \{v\in V(G_i)\setminus D_i | dist_{G_i}(v, Q) > d_{min} \}$. We have two importantly useful observations as follows. 

\squishlisttight

\item For each vertex $v\in S_u$, we need to recompute the query distance $dist_{G_{i+1}}(v, Q)$. It is due to the fact that the vertex $u$ with $dist_{G_{i}}(u, Q) <= d_{min}$ keeps the query distance unchanged in $G_{i+1}$. This is because no vertices that are along with the shortest paths between $u$ and $Q$, are deleted in graph $G_{i}$. 

\item For vertex $v\in S_u$, $dist_{G_{i+1}}(v, Q) \geq dist_{G_{i}}(v, Q)$ always holds, due to $G_{i+1} \subseteq G_{i}$. Thus, instead of traversing from query nodes $Q$, we update the query distance  $dist_{G_{i+1}}(v, Q)$ by traversing from $S_s$, where $S_s = \{v\in V(G_i)\setminus D_i | dist_{G_i}(v, Q) = d_{min} \}$.
\end{list}


% We claim the nodes set we need to update is $S_u = \{n_i | distance(n_i, q) > d \}$. The reason is the nodes that hold $distance \leq d$, their shortest path won't change because the nodes on their shortest path haven't been deleted, i.e. not in $S$. Another key observation is that for the nodes in $S_u$, their shortest path to $q$ won't become smaller since we only delete nodes from the graph but not adding any edges to the graph. So now we will start running BFS from the nodes set $S_s = \{n_i | dist(n_i, q) = d \}$ in the BFS manner but not like the naive method starting from $q$ to search the whole graph, which could significantly reduce the search space.

% To be more specific in our problem, since we have two query nodes, without loss of generality, let's assume the value of $dist_{G_l} (G_l, Q)$ in line \ref{line:a6} of Algorithm~\ref{algo:Basic} is determined by nodes set $S$ to $q_l$, then influenced nodes $S_u = \emptyset$ for $q_l$ since $S$ are the nodes farthest to $q_l$. Then we don't need to compute the shortest path on graph $G$ to $q_l$. But due to the asymmetric topological structure of $q_l$ and $q_r$ on the graph, the distance of the deletion nodes $S$ are not farthest to $q_r$ or even with different shortest path values to $q_r$, the searching start set $S_s$ is determined by the value of $min_{u \in S} dist(u, q_r)$. In practice the inner distance $l$ between query nodes $q_l$ and $q_r$ will influence the size of $S_u$. The details of the algorithm (set $q = q_r$) are as follows.

%Actually $\for u\in S_u$, $dist(u, Q) = dist(v, Q) + dist(u, v) = d_{min} + dist(u,v)$ where $v \in S_s$. We save the time to compute $dist(v, Q)$ which is $d_{min}$ and only need update $dist(u,v)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\small
\caption{Leader Pair Identification $(G, q)$} \label{algo:LeaderPair}
\begin{algorithmic}[1]
\REQUIRE A graph $G = L$ (or $R$), a query node $q = q_l$ (or $q_r$)
\ENSURE A lead node $p=v_l$ (or $v_r$);
%\STATE $p \gets argmax_{v \in G} \chi(v)$;
\STATE $p \gets q$;
%\IF{dist$(p, q) \leq d_p$}
%    \STATE return $p$;
\STATE $b_{max} \gets max_{v \in G} \chi(v)$;
\IF{$\chi(v) > b_{max}/2$}
    \STATE return $p$;
\ELSE
    \STATE $b_p \gets b_{max}/2$;
    \WHILE{$b_p > b$}
        \STATE $d \gets 1$;
        \WHILE{$d < b_p$}
            \STATE $S \gets \{u|dist_{G} (u, q) = d, u \in G\}$; \label{line:a11}
            % \FOR{$s \in S$}
            %     \IF{$\chi(s) \geq b_p$}
            %         \STATE $p \gets s$;
            %         \STATE break;
            %     \ENDIF
            % \ENDFOR
            \IF{$\exists s \in S$ that $\chi(s) \geq d_p$} \label{line:a12}
                \STATE return $s$; \label{line:a13}
            \ELSE \label{line:a13}
                \STATE $d \gets d + 1$; \label{line:a14}
            \ENDIF
        \ENDWHILE
        \STATE $b_p \gets b_p/2$; \label{line:a15}
    \ENDWHILE 
\ENDIF
\STATE return $p$; \label{line:a16}
\end{algorithmic}
\end{algorithm}


We present the method of fast query distance computation in Algorithm~\ref{algo:sssp}. First, we remove a set of nodes $D_i$ from graph $G_i$ (line \ref{line:a1}). We then calculate the minimum distance $d_{min}$, which is the minimum length of the shortest path from $D_i$ to $q$ (line \ref{line:a2}). We select nodes $S_s$ whose shortest path equals to $d_{min}$ (line \ref{line:a3}) as the BFS starting points . Let a set of nodes to be updated as $S_u$ whose shortest path is larger than $d_{min}$ (lines \ref{line:a4}). Then, we run the BFS algorithm starting from nodes in $S_u$, we treat $S_u$ as unvisited and all the other nodes as visited (line \ref{line:a5}). The algorithm terminates until $S_u$ are visited or BFS queue becomes empty. Finally, we return the shortest path to $q$ for all vertices (line \ref{line:a6}).

%Two hashtables are updated by removing the deleted nodes $S$ (lines \ref{line:a3}-\ref{line:a4}).

%In the minimizing diameter settings for any node in $V$ the shortest path to $q$ will be the same, denoted by $d$. So we could get $d$ from $dist$ by return the value of any node in $V$ (line \ref{line:a2}).


% \begin{algorithm}[t]
% \small
% \caption{Fast Query Distance Computation$(G, q, S, dist, hm)$} \label{algo:sssp}
% \begin{algorithmic}[1]
% \REQUIRE A graph  $\mathcal{G} = (V, E)$, query node $q$, deletion nodes set $V$
% \ENSURE $dist, hm$
% \STATE remove $S$ form $G$;
% %\STATE $d = dist(S.iterator.next())$;
% \STATE $d \gets min_{u \in S} dist(u, q)$;
% \FORALL{$v \in S$}
%     \STATE $dist.remove(v)$; $hm[dist[v]].remove(v)$;
% \ENDFOR
% \STATE $S_u \gets \emptyset$;
% \FORALL{$i \in hm.keys()$ and $i > d$}
%     \STATE $S_u \gets S_u \cup \{hm[i]\}$;% mark S_u as unvisited
% \ENDFOR
% \STATE $Q \gets queue$;
% \STATE $S_s \gets hm[d]$;
% \FORALL{$s \in S_s$}
%     \STATE $Q.enqueue(s)$; \label{line:a11}
% \ENDFOR
% \WHILE{$Q \neq \emptyset$} \label{line:a12}
%     \STATE $v \gets Q.dequeue()$; \label{line:a13}
%     \FORALL{$w \in N(v)$} \label{line:a14}
%         \IF{$w \in S_u$} \label{line:a15}
%             \STATE $Q$.enqueue(w); \label{line:a16}
%             \STATE $dist[w] \gets dist[v] + 1$; \label{line:a17}
%             \STATE $hm[dist[w]].add[w]$; \label{line:a18}
%             \STATE $S_u.remove(w)$; \label{line:a19}
%             \IF{$S_u == \emptyset$} \label{line:a20}
%                 \STATE break; \label{line:a21}
%             \ENDIF
%         \ENDIF
%     \ENDFOR
% \ENDWHILE
% \STATE return $dist$, $hm$; \label{line:a22}
% \end{algorithmic}
% \end{algorithm}


\subsection{Leader Pair Identification}\label{sub-sec:lp}
%Leader Pair Identification for reducing butterfly counting.
In this subsection, we present efficient algorithms for leader pair identification, which can reduce the butterfly counting. 



\spara{Leader Pair Identification}. The butterfly counting in Algorithm~\ref{algo:count} needs to be invoked once a graph $G_i$ is updated in Algorithm~\ref{algo:Basic}. This may lead to a large number of butterfly counting, which is very time costly. Recall that the definition of BCC, it requires a pair of nodes $(v_l\in L, v_r \in R)$ such that   $\chi(v_l) \geq b$ and $\chi(v_r) \geq b$. This motivates us to find a good pair  of leader vertices, whose butterfly degrees are large enough w.r.t. $b$  in two groups $L$ and $R$, even after a number of graph removal iterations. Thus, it can avoid to find a new leader pair and save the time cost. In the following, we show two key observations to find a good leader pair $P(v_l, v_r)$ where $v_l\in L$ and $v_r \in R$.

\begin{observation}
The leader pair $P$ should have large butterfly degrees $\chi(v_l)$ and $\chi(v_r)$, which do not easily violate the constraint of cross-over interactions.  
\end{observation}

\begin{observation}
The leader pair $P$ should have small query distances $dist(v_l, Q)$ and $dist(v_r, Q)$, which are  close to query nodes $Q$ and not easily deleted by graph removal.
\end{observation}

%We set a threshold $b_p \gg b$, we select the value $b_p$ in a quantile way, i.e. the butterfly number of p\% of the nodes in the bipartite graph is less than $b_p$. Then we proposed a simple strategy to find the leader pair in algorithm~\ref{algo:LeaderPair}.


%need to discuss heap top butterfly count candidates set.
\begin{algorithm}[t]
\small
\caption{Butterfly Degree Update for Leader Pair $(G, p, v)$} \label{algo:UpdatePair}
\begin{algorithmic}[1]
\REQUIRE A graph $B = (V, E)$, an leader node $p$, a deletion node $v$
\ENSURE $\chi(p)$
%\STATE $count \gets 0$;
\IF{$\ell(v) = \ell(p)$}
    % \FOR{$s \in N(p)$}
    %     \IF{$s \in N(v)$}
    %         \STATE $count \gets count + 1$;
    %     \ENDIF
    % \ENDFOR
    \STATE $cn \gets |n_{pv}|$;
    \STATE $\chi(p) \gets \chi(p) - C_{cn}^{2}$;
\ELSE
    \IF{$v \in N(p)$}
        \FOR{$s \in N(p)$}
            % \FOR{$u \in N(v)$}
            %     \IF{$u \in N(s)$}
            %         \STATE $cn \gets cn + 1$;
            %     \ENDIF
            % \ENDFOR
            \STATE $cn \gets cn + |n_{vs}|$;
        \ENDFOR
        \STATE $\chi(p) \gets \chi(p) - cn$;
    \ENDIF
\ENDIF
\STATE return $\chi(p)$;
\end{algorithmic}
\end{algorithm}


We present the algorithm of leader pair identification in Algorithm~\ref{algo:LeaderPair}. Here, we use the graph $G$ to represent a group graph $L/R$ and find a lead node $v_l/v_r$. We first initiate $p$ as the query node $q$ since it's the closest with distance $0$ (line \ref{line:a1}). This is especially effective when the input query node is leader biased who contain the largest butterfly degree. If the degree number is large enough, i.e., greater than $b_{max}/2$, we return $p$ as the leader node (\ref{line:a3}-\ref{line:a4}); Otherwise, we find the leader node $p$ in the following manner. We first vary $d$ from $1$ to $d_p$, and decrease $b_p$ in $\{b_{max}/2, b_{max}/4, ..., b\}$ (line \ref{line:a6}, \ref{line:a15}). We compute a set of nodes $S$ whose distance to the query is $d$ (line \ref{line:a10}). Then, we identify one vertex $s\in S$ with $\chi(s)\geq b_p$ and return as the leader node otherwise we increase $d$ by $1$ to search the next hop (lines \ref{line:a11}-\ref{line:a14}). %If $p$ does not exist, then we increase $d$ by $1$(line \ref{line:a15}). If not find in the value $b_p$, we divide it by $2$ to the next loop (line \ref{line:a16}).
Note that we return an initial $p$ if no better answer is identified (line \ref{line:a16}).
% The time complexity of the algorithm~\ref{algo:LeaderPair} is $O(n)$ since for one node the running cost is $O(1)$ and the worst case is iterating all the nodes.

% distance $dist(p,q)$ is no greater than a given proximity parameter $d_p$, we return $p$ as the leader node 



% \begin{algorithm}[t]
% \small
% \caption{LeaderPair$(G)$} \label{algo:LeaderPair}
% \begin{algorithmic}[1]
% \REQUIRE A graph  $\mathcal{G} = L \cup R$, a set of nodes to be removed as $S$
% \ENSURE A leader pair $P = (p_l, p_r)$
% \STATE $b_p \gets b_{max}/2$;
% \STATE $b_p \gets b_{max}/2$;
% \WHILE{$b_p > b$}
%     \STATE Initialize $P = (p_l, p_r) \gets (q_l, q_r)$;
%     \FORALL{$p \in P$}
%         \STATE $d = 1$;
%         \WHILE{butterfly[p] $< b_p$}
%             \IF{$\ell(p) == \ell(q_l)$}
%                 \STATE $sub \gets L$; $q \gets q_l$;
%             \ELSIF{$\ell(p) == \ell(q_r)$}
%                 \STATE $sub \gets R$; $q \gets q_r$;
%             \ENDIF
%             \STATE $S \gets \{u|dist_{sub} (u, q) = d, u \in sub\}$;
%             \FORALL{$s \in S$}
%                 \IF{butterfly[s] $\geq b_p$}
%                     \STATE $p = s$;
%                     \STATE break;
%                 \ENDIF
%             \ENDFOR
%             \STATE $d = d + 1$;
%         \ENDWHILE
%     \ENDFOR
%     \STATE $b_p \gets b_p/2$;
% \ENDWHILE
% \STATE return $P$;
% \end{algorithmic}
% \end{algorithm}

\spara{Butterfly Degree Update for Leader Pair}. Here, we consider how to efficiently update the butterfly degrees $\chi(v_l)$ and $\chi(v_r)$ after graph removal in Algorithm~\ref{algo:Basic}. 

The algorithm of updating the butterfly degrees of leader pair is outlined in algorithm~\ref{algo:UpdatePair}. First, we check the labels of $v$ and $p$ (line \ref{line:a1}). If $\ell(v) = \ell(p)$,  we calculate the common neighbors of $p$ and $v$, i.e., $cn$ and the number of butterflies containing $p$ and $v$ is $C_{cn}^{2}$. Then,  $\chi(p)$ decreases by $C_{cn}^{2}$ (lines \ref{line:a3}-\ref{line:a4}). If $\ell(v) \neq \ell(p)$, we enumerate each vertex $u$, i.e., $v$'s neighbors, and check the common neighbors of them with $p$. Note that $cn$ keeps the number of butterflies involving $v$, so we directly update $\chi(p)$  by decreasing $cn$ (lines \ref{line:a6}-\ref{line:a9}).
% %we need to check if the deletion node $v$ is on the same or different side with $p$ since the algorithm will be different  
 %For the same side,

% \begin{algorithm}[t]
% \small
% \caption{UpdatePair$(G, P)$} \label{algo:UpdatePair}
% \begin{algorithmic}[1]
% \REQUIRE A graph $G = (V, E)$, leader node $P$, deletion node $v$
% \ENSURE
% \FORALL{$p \in P$}
%     \STATE $count = 0$;
%     \IF{$\ell(v) == \ell(p)$}
%         \FORALL{$s \in N(p)$}
%             \IF{$s \in N(v)$}
%                 \STATE $count = count + 1$;
%             \ENDIF
%         \ENDFOR
%         \STATE $\chi(p) \gets \chi(p) - C_{count}^{2}$;
%     \ELSE
%         \FORALL{$s \in N(p)$}
%             \FORALL{$u \in N(v)$}
%                 \IF{$u \in N(s)$}
%                     \STATE $count \gets count + 1$;
%                 \ENDIF
%             \ENDFOR
%         \ENDFOR
%         \STATE $\chi(p) \gets \chi(p) - count$;
%     \ENDIF
% \ENDFOR
% \STATE return;
% \end{algorithmic}
% \end{algorithm}

\spara{Complexity analysis}. Next we analyze the time complexity of leader pair strategy which consists of Algorithm~\ref{algo:LeaderPair} and ~\ref{algo:UpdatePair}. 

\begin{theorem}
The total complexity of leader pair strategy is $O(n + d_v d_r)$.
\end{theorem}

\spara{Proof Sketch:} Assume that the degree of $v_l$ and $v_r$ in graph $B$ are $d_l$, $d_r$ respectively and the degree of deleted node $v$ is $d_v$. The time complexity of Algorithm~\ref{algo:UpdatePair} is $O(min(d_p, d_v))$ if $\ell(v) = \ell(p)$;  The time complexity of Algorithm~\ref{algo:UpdatePair} is $O(d_v d_p)$ if $\ell(v) \neq \ell(p)$. Thus, the total complexity of Algorithm~\ref{algo:LeaderPair} and ~\ref{algo:UpdatePair} is $O(n + d_v d_r)$. It's much more efficiency than Algorithm~\ref{algo:count}, which takes $O(\sum\nolimits_{u \in L \cup R} {d_u^2} )$ time. 


% To further improve the efficiency, we design an upper bound for updating butterfly degree. That is, 

% \begin{observation}
% When delete one node $v$ whose degree denoted as $d_v$ and assume it's in the same side with $p_l$, the upper bound of butterfly number it form with the leader node is: for same side it's $C_{min(d_v, d_l)}^{2}$; for different side it's $(d_v - 1)(d_r - 1)$.
% \end{observation}

%%%%%%
\begin{algorithm}[t]
\small
\caption{LocBCC $(G, Q)$} \label{algo:locbcc}
\begin{algorithmic}[1]
\REQUIRE  A graph $G = (V, E, \ell)$, query nodes $Q = \{q_l, q_r\}$.
\ENSURE A connected $(k_1, k_2, b)$-BCC $R$ with a small diameter.
\STATE Compute a Steiner tree $T$ connecting $Q$ using butterfly-core distance as edge weight;
\STATE $k_l \gets \min_{v \in L} \delta(v)$; $k_r \gets \min_{v \in R} \delta(v)$;
\STATE Iteratively expand $T$ into graph $G_t = \{v \in L | \delta(v) \leq k_l \} \cup \{v \in R | \delta(v) \leq k_r \}$ by adding adjacent vertices $v$, until $|V(G_t)| > \eta$;
\STATE Compute a connected $(k_1, k_2, b)$-BCC containing $Q$ of $G_t$ with the largest coreness on each side;
\STATE Apply a variant of BulkDelete algorithm on $G_t$ to identify the final BCC
\end{algorithmic}
\end{algorithm}
\vspace{-2mm}


\subsection{Index-based Local Exploration}\label{sub-sec:lc}
In this section, we develop a query processing algorithm which efficiently detects a small neighborhood subgraph candidate around query vertices $Q$, which tends to be densely connected both in its own label subgraph and the bipartite graph.
%In this section, we develop a heuristic strategy to quickly find the BCC by local exploration, which finds a small candidate graph of BCC in the local neighborhood of the query vertices 𝑄.

First, we construct the BCindex for all vertices in $G$. The data structure of BCindex consists of two components: the coreness and butterfly number. For $k$-core index construction of each vertex, we apply the existing core decomposition \citep{batagelj2003m} on graph $G$ to construct its coreness. The $k$-core has a nested property, i.e., the $k_1$-core of graph $G$ must be a subgraph of $k_2$-core of graph $G$ if $k_1 > k_2$. The offline $k$-core index could efficiently find $k$-core subgraphs from $G$, meanwhile filter out disqualified edges $\{e = (v_i, v_j) \in B |\delta(v_i) < k_1$ or $\delta(v_j) < k_2 \}$ in the bipartite graph $B$. Moreover, we keep the butterfly degree number index of each vertex on the bipartite graph with different labels using Algorithm~\ref{algo:count}.

Based on the obtained BCindex, we present our method of index-based local exploration, the algorithm starts from the query vertices, and finds a minimal Steiner tree connecting the two query vertices, which is a well-known NP-hard problem but admitting $2$-approximation to optimal solutions \citep{kou1981fast} \citep{wu1986faster}. A naive method is to find a minimal weight Steiner tree to connect all query vertices, where the weight of a tree is the number of edges, while this may produce a result with a small coreness and butterfly degrees. To this end, we define a weighted distance for a path $P$ between $u$ and $v$ as follows.

\begin{definition}[Butterfly-Core Distance]
Given an edge $e = (u,v) in G$, the butterfly-core distance is defined as $\underline{dist}(u, v) = dist_G(u,v) + \gamma_1 (\delta_{max} - \min_{v \in P} \delta(v)) + \gamma_2 (\chi_{max} - \min_{v \in P}\chi(v))$, where $\delta(v)$ is the coreness of vertex $v$, $\chi(v)$ is the butterfly degree of $v$, $\delta_{max}$ and $\chi_{max}$ are the maximum coreness and the maximum butterfly degree in $G$.
\end{definition}
\vspace{-2mm}

The difference $(\delta_{max} - \min_{v \in P} \delta(v))$ and $(\chi_{max} - \min_{v \in P}\chi(v))$ measures the shortfall in the coreness and butterfly degree of edge $e$ w.r.t. the corresponding maximum value in $G$. Here $\gamma_1$ controls the extent to which a small node coreness is penalized, $\gamma_2$ controls the extent to which a small butterfly degree is penalized. We then expand the extracted tree to a graph $G^{'}$ by involving the local neighborhood of query nodes. Based on $G^{'}$, we find a connected BCC with the highest $k_1$ and $k_2$ containing $Q$, and then iteratively remove the furthest nodes from this BCC. Moreover, to reduce the iteration number of butterfly-core maintenance, we propose to delete a batch of nodes with the same furthest query distance, which can further improve the search efficiency. Furthermore, we construct an offline $k$-core index for efficiently find $k$-core subgraphs from $G$.


